Don't Classify, Translate: Multi-Level E-Commerce Product Categorization Via Machine Translation

E-commerce platforms categorize their products into a multi-level taxonomy tree with thousands of leaf categories. Conventional methods for product categorization are typically based on machine learning classification algorithms. These algorithms take product information as input (e.g., titles and descriptions) to classify a product into a leaf category. In this paper, we propose a new paradigm based on machine translation. In our approach, we translate a product's natural language description into a sequence of tokens representing a root-to-leaf path in a product taxonomy. In our experiments on two large real-world datasets, we show that our approach achieves better predictive accuracy than a state-of-the-art classification system for product categorization. In addition, we demonstrate that our machine translation models can propose meaningful new paths between previously unconnected nodes in a taxonomy tree, thereby transforming the taxonomy into a directed acyclic graph (DAG). We discuss how the resultant taxonomy DAG promotes user-friendly navigation, and how it is more adaptable to new products.

==> result.tex <==
\section{Results}
\label{sect:result}

\begin{table}[H]
    \begin{tabular}{l|l|ccc|ccc}
    ~                       & ~                         &  ~  & \textbf{RDC}     & ~     & ~ &  \textbf{Ichiba}     & ~     \\
    ~                       & ~                         & \textbf{P}     & \textbf{R}     & \textbf{F}     & \textbf{P}      & \textbf{R}     & \textbf{F}     \\ \hline
                  & \textbf{Deep Belief Net (DBN)}     & 72.19 & 74.72 & 72.86 & 78.09  & 78.29 & 77.52 \\
    \texttt{CUDeep}                & \textbf{K-Nearest Neighbors (KNN)} & 71.14 & 72.10 & 70.94 & 79.24  & 78.69 & 78.66 \\
                   & \textbf{DBN + KNN}                 & 73.46 & 75.57 & 73.85 & 82.65  & 82.27 & 82.05 \\ \hline
    ~                       & \textbf{RNN Seq2Seq  (RNN)}        & 74.03 & 73.43 & 72.50 & 84.70   & 82.39 & 82.08 \\

Ours                    & \textbf{Transformer Seq2Seq}       & 74.44 & 75.25 & 73.83 & 83.79  & 83.59 & 84.74 \\
    ~                       & \textbf{RNN + Transformer }        & \textbf{75.22} & \textbf{75.65} & \textbf{74.19} & \textbf{85.08}      & \textbf{84.31}     & \textbf{84.26}     \\
    \end{tabular}
\caption{Results of our NMT Systems vs \texttt{CUDeep} Classification Systems}
\label{tb:results}
\end{table}

\begin{table}[H]
\begin{center}
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
    &	\multicolumn{6}{c}{RDC} & \multicolumn{6}{c}{Ichiba} \\
     & \multicolumn{3}{c}{\textbf{p5}} & \multicolumn{3}{c}{\textbf{p95}} & \multicolumn{3}{c}{\textbf{p5}} &	\multicolumn{3}{c}{\textbf{p95}}\\
   \textbf{Model} & \textbf{P} &	\textbf{R} &	\textbf{F} & \textbf{P} &	\textbf{R} &	\textbf{F}& \textbf{P} &	\textbf{R} &	\textbf{F}& \textbf{P} &	\textbf{R} &	\textbf{F} \\ \hline
    DBN + KNN & 73.08 & 75.17 & 73.32 & 74.11 & 75.98 & 74.22 \\
    RNN + Transformer & 74.81 & 75.23 & 73.68 & 75.76 & 76.05 &74.57 \\
    \end{tabular}
\caption{Confidence Interval of 1000 iterations of Bootstrap Resampling on the Best Performing Models}
\label{tb:bootstrap-results}
\end{center}
\end{table}

\begin{table}[H]
\begin{center}
    \begin{tabular}{l|ccc|rrr}
    			&		\multicolumn{3}{c}{Average} & \multicolumn{3}{c}{Variance} \\
    \textbf{Model} &	\textbf{P} &	\textbf{R} &	\textbf{F}	& \textbf{P} &	\textbf{R} &	\textbf{F} \\ \hline
    RNN & 74.58 & 73.18 & 72.66 & \textbf{0.1374} & \textbf{0.1888} & \textbf{0.1874}\\
    Transformer & 75.54	& 74.14 & 73.22 & 0.5703 & 1.609 & 1.958\\
    RNN + Transformer & \textbf{76.66} & \textbf{76.14} &	\textbf{75.14} & 0.3142 & 0.8065 & 1.064\\
    \end{tabular}
\caption{NMT system's Stratified 4-fold Cross-Validation Results on RDC Dataset}
\label{tb:cross-val-results}
\end{center}
\end{table}

Table-~\ref{tb:results} presents the evaluation results held-out test set as described in the Section 4.1. Generally, our Transformer model outperforms all \texttt{CUDeep} single models on both datasets at 73.83 F-score for the RDC test set and 84.74 F-score for the Ichiba held-out test set. While \texttt{CUDeep} DBN + KNN ensemble outperform our single Transformer model marginally on the RDC, our RNN + Transformer ensemble model outperfoms \texttt{CUDeep} in both datasets and achieves the highest weighted precision, recall and F-score on all accounts. 

To further confirm that our system outperforms \texttt{CUDeep}, we conducted 1000 iterations of bootstrap resampling on the best performing model in each system to find out the 95\% confidence interval of their performance scores.
We present the results in Table-~\ref{tb:bootstrap-results}.


We also carried out stratified 4-fold cross validation on the RDC dataset \footnote{Due to computational resource constraints, we did not manage to carry out the stratified 4-fold cross validation on the Ichiba dataset.}. The average and variance of the weighted precision, recall and F1 score across the folds are shown in Table-~\ref{tb:cross-val-results}. We can observe from the variance across the folds that the Transformer model has larger variability than the RNN model. The ensemble of them still achieves the best results








